Memory Efficient Patch-based Training for INR-based GANs

Recent studies have shown remarkable progress in GANs based on implicit neural representation (INR) - an MLP that produces an RGB value given its (x, y) coordinate. They represent an image as a continuous version of the underlying 2D signal instead of a 2D array of pixels, which opens new horizons for GAN applications (e.g., zero-shot super-resolution, image outpainting). However, training existing approaches require a heavy computational cost proportional to the image resolution, since they compute an MLP operation for every (x, y) coordinate. To alleviate this issue, we propose a multi-stage patch-based training, a novel and scalable approach that can train INR-based GANs with a flexible computational cost regardless of the image resolution. Specifically, our method allows to generate and discriminate by patch to learn the local details of the image and learn global structural information by a novel reconstruction loss to enable efficient GAN training. We conduct experiments on several benchmark datasets to demonstrate that our approach enhances baseline models in GPU memory while maintaining FIDs at a reasonable level.

==> backup.tex <==
\iffalse
\subsection{Failure on naive patch training}
\yj{이 section은 experiment에서 설명하는게 좋을것 같아요}
The most common way to train GAN memory efficiently is using a patch discriminator that is already used in image-to-image translation.
Particularly, since INR-based GAN can generate only patches for discrimination through coordinate sampling at the generator (see (x,y) at Stage 3 in Fig. 2), GPU memory can be reduced in proportion to the size of the generated patch.

However, unlike the results in image-to-image translation, results in image generation are very disappointing.
They lack the overall structural information, which is caused by the generator learning the local texture detail through the patch discriminator, but no proper learning signal was injected into the generator for the global coherence.
\fi


\iffalse
\subsection{Multi-stage patch training}
\yj{삭제. section 2.2로 옮기기}
We propose multi-stage patch training as a way to learn global structural information in the training process to resolve the failure of patch training.
Multi-stage patch training consists of three stages.

\textbf{1st Stage,}
we sparsely sample coordinates of a resolution corresponding to 1/4 (ex. 2x2) of our final resolution (ex. 8x8) in the coordinate space and input them together with latent to the generator, and use image discriminator's adversarial loss for training.

loss 수식. (adversarial loss를 그냥 Ladv라고 써도 되는지? 아니면 일일이 풀어서 다 써야하나)

In the 1st stage, the generator cannot learn the local detail of the final resolution image, but it is possible to learn about the overall structure of the image by full image discrimination even though it has a low resolution.

\textbf{2nd Stage,}
we sparsely sample coordinates of a resolution corresponding to 1/2 (ex. 4x4) of our final resolution (ex. 8x8) in the coordinate space, randomly crop corresponding to 1/4 (ex. 2x2)  of our final resolution (ex. 8x8), and input them together with latent to the generator.
Also, a novel \textbf{reconstruction loss} is applied for maintaining global consistency.
(여기 사실 어떻게 풀어서 써야할지 잘 모르겠습니다... coordinate smapling을 알맞은 위치에 2개 다 한다음에 같은 latent를 넣어서 image를 생성하고, align 시켜서 downsampling한다음에 reconstruction한다는 내용)
We use patch discriminator's adversarial loss and reconstruction loss jointly for training.

loss 수식.

From the 2nd stage, it is very difficult for the generator to learn information about the overall structure of the image because the discriminator does not use the entire image, but only look at the patch of the image to descriminate.
The reconstruction loss was introduced to solve this problem, which can resolve for the problem the patch discriminator by restoring the image generated by previous stage's generator which learned the overall structure of the image well in the 1st stage.

\textbf{3rd Stage,} except for we sample coordinates of our final resolution (ex. 8x8) and randomly crop to 1/4 (ex. 2x2) of our final resolution, the whole training process is same as 2nd Stage, and use patch discriminator's adversarial loss and reconstruction loss for training.

loss 수식.

As described above, with multi-stage patch training, memory efficient training is possible because the size of the image generated during training does not exceed 1/4 of the final resolution.
\fi

\subsection{Design space of learned constant initialization}
\yj{이건 굳이 설명할 필요 있을까요? 저희 contribution으로 볼 수 있나요?}
CIPS uses learned constant in addition to implicit neural representation for generator's positional encoding.
During multi-stage patch training, implicit neural representation can use sampled coordinates as inputs for each stage, but the learned constant should be newly initialized because it has fixed resolution.
Below are several choices we have for learned constant initialization.

- Random: we randomly initialize the learned constant at each stage.

- Nearest Neighbor: we initialize the learned constant by nearest neighbor upsampling from last stage's learned constant.

- Bilinear: we initialize the learned constant by bilinear upsampling from last stage's learned constant.

- Remove: we do not use the learned constant for training (just using implicit neural representation for positional encoding).

We conduct empirical experiments on several benchmark datasets for exploring the effect of various initialization strategies to final training results (see Sec. 3-4).

